World Action Modeling with Progressive Visual Planning

World action models (WAMs) have emerged as a promising paradigm for robotic control by jointly predicting future visual dynamics and actions from an initial observation and instruction. However, existing WAMs struggle with long-horizon prediction, as generating dense video rollouts is highly inefficient. Some recent WAMs address this by predicting a single future frame without generating the full video, but this approach neglects how to progress toward the goal. We present ProWAM, a progressive world action model that jointly predicts actions and an ordered sequence of sparse visual sub-goals, providing explicit visual guidance to anchor action generation throughout task execution. This design scales naturally, as sub-goal prediction can be learned from large-scale action-free videos, allowing the video backbone to offload complex visual planning from the action policy. For efficient action generation, ProWAM executes a single video-backbone forward pass to cache sparse sub-goal features, eliminating iterative full-video generation and requiring only lightweight action denoising during replanning. Across extensive evaluations, ProWAM achieves superior out-of-distribution robustness. On simulation benchmarks, it sets new state-of-the-art results on LIBERO-Plus (85.8%) and randomized RoboTwin (75.7%), outperforming the strongest baseline with relative gains of up to +35.9%. On RoboCasa365, ProWAM achieves a 48.1% success rate and 18.2% on the challenging Composite-Unseen split, ranking 4th overall. Crucially, in zero-shot real-world experiments, ProWAM achieves 70.0% success, outperforming the strongest baseline by +15.0 (from 55.0% to 70.0%, a +27.3% relative gain) in novel scenes. These results demonstrate the value of progress-indexed visual foresight for closed-loop control. Our program is in https://sii-ferenas.github.io/ProWAM-page.

==> sections/method.tex <==
\section{Method}\label{sec_method}
\subsection{Simple Sub-goal Leads Better Policy}
\subsection{ProWAM: Making Progressive Planning for Better}



\paragraph{Efficient inference via sub-goal KV-caching.}
Rather than the burdensome joint denoising that advances the video and action branches at a shared pace—re-invoking the heavy video expert at a common $T$ steps, we exploit the observation that a \emph{single} denoising step already
yields a sub-goal with the correct target configuration, as further refinement only adds texture the action head ignores.
We thus invoke the video expert \emph{once} to generate and cache the sub-goal's
key/value features, then denoise the action head against this cache, because the
sub-goal is conditioned on the fixed observation $f_0$ it is constant across
action steps, making the single cache exact.
This cuts video-expert forwards from $T$ to $1$ ($\sim$10$\times$), matching the
cost of~\cite{pai2025mimic,yuan2026fastwam,zhang2026imagewam} with no accuracy loss (refer to Appendix~\ref{sec:kvcache} for further details).

